Beyond the Black Box: A Statistical Model for LLM Reasoning and Inference

This paper introduces a novel Bayesian learning model to explain the behavior of Large Language Models (LLMs), focusing on their core optimization metric of next token prediction. We develop a theoretical framework based on an ideal generative text model represented by a multinomial transition probability matrix with a prior, and examine how LLMs approximate this matrix. Key contributions include: (i) a continuity theorem relating embeddings to multinomial distributions, (ii) a demonstration that LLM text generation aligns with Bayesian learning principles, (iii) an explanation for the emergence of in-context learning in larger models, (iv) empirical validation using visualizations of next token probabilities from an instrumented Llama model Our findings provide new insights into LLM functioning, offering a statistical foundation for understanding their capabilities and limitations. This framework has implications for LLM design, training, and application, potentially guiding future developments in the field.

==> Dirichlet_Approx.tex <==
\section{Dirichlet approximation}
We now show that any prior over multinomial distributions can be approximated as a finite mixture of Dirichlet distributions.

\begin{theorem}[{Dirichlet approximation}] \label{thm:dirichlet} Any distribution over $multinomial$ probabilities \\ $u(p_{1},p_{2},\cdots p_{m})$ which has a continuous bounded density function can be approximated as a finite mixture of Dirichlet distributions. 
\end{theorem}
\begin{proof} 
Consider a multinomial distribution on probabilities $P=(p_1,p_2,\cdots ,p_m), \sum p_i =1.$ Now consider a fictitious experiment of generating $n$ observations from this multinomial distribution resulting in $x_i$ observations in $i^{th}$ category, $i=1,2,\cdot m$. Note that $x_i \geq 0, i=1,\cdots,m$ and $\sum_i x_i =n$. Let $(\hat{P_n})=(x_1, x_2,\cdots ,x_m)/n)$, be the corresponding empirical probabilities. 

Then by the strong law of large numbers, $\hat{P_n} \rightarrow P \, a.s.$ Then, for any bounded continuous function, $$E(u((\hat{P_n})) \rightarrow u(P) \, \mbox{uniformly in} \, P. \, \mbox{where },$$ 
\begin{align*}
E(u(\hat{P_n})) &= \sum_{x_1,\dots ,x_m} u\left(\frac{x_1}{n},\frac{x_2}{n}, \dots, \frac{x_m}{n}\right) \\
&\quad \times \frac{\Gamma(n+1)}{\Gamma(x_1+1)\cdots\Gamma(x_m+1)} \prod_{i} p_i^{x_i}
\end{align*}

Now let ${\mathcal{D}}(p|\alpha_1,\alpha_2,\dots ,\alpha_m)$ be a the density of an $m$ Dirichlet distribution with parameters $\alpha_1,\alpha_2,\dots ,\alpha_m$. Then, the above can be simplified to show that:
\begin{align*}
E(u(\hat{P_n})) &= \sum_{x_1,\dots ,x_m} u\left(\frac{x_1}{n},\frac{x_2}{n}, \dots, \frac{x_m}{n}\right) \\
&\quad \times \frac{\Gamma(n+1)}{\Gamma(n+m)} \mathcal{D}(p|x_1+1,x_2+1,\dots ,x_m+1) \\
&\quad \rightarrow u(p)
\end{align*}


However, since $\int u(p) dp =1$, the integral of the middle term above  also tends to $1$. Using this fact and normalizing it gives us:
\begin{align*}
\sum_{x_1,\dots ,x_m} &u^{*}\left(\frac{x_1}{n},\frac{x_2}{n}, \dots, \frac{x_m}{n}\right) \\
&\times \mathcal{D}(p|x_1+1,x_2+1,\dots ,x_m+1) \rightarrow u(p)
\end{align*}
\text{where, }
\begin{align*}
u^{*}\left(\frac{x_1}{n},\frac{x_2}{n}, \dots, \frac{x_m}{n}\right) &= \frac{u\left(\frac{x_1}{n},\frac{x_2}{n}, \dots, \frac{x_m}{n}\right)}{\sum_{x_1,\dots ,x_m} u\left(\frac{x_1}{n},\frac{x_2}{n}, \dots, \frac{x_m}{n}\right)}
\end{align*}

\end{proof}


The theorem is more general with appropriate regularity conditions. The convergence under the above conditions is in $L_1$ as well as in Total Variation in $p$ and the posteriors also converge. A special case of this is $Binomial$ distribution with $Beta$ prior, whereby any arbitrary prior for Binomial distribution can be approximated by a mixture of Beta distributions. Similar results apply to the general exponential family and for approximating a random probability measure by the mixtures of Dirichlet Processes~\cite{dalal1980approxMDP}.
\begin{comment}
    

Estimating arbitrary $u(p_{1},p_{2},\cdots p_{m})$ is difficult. The above theorem allows us to approximate each such distribution by a mixture of known Dirichlet distributions, with unknown mixing constants. These can be then determined by EM type algorithm. 

\end{comment}

Theorem~\ref{thm:dirichlet} can lead to an efficient design of LLMs by identifying a small "basis set" by which any arbitrary $Multinomial$ distribution can be generated. It can help identify the right training set for a particular task that enables the creation of this basis set. Current practice of training LLMs is to use a mildly curated version of ``the Internet" (wikipedia, reddit posts etc.) and a rigorous way to create the training set is needed.



==> Extra_fewshot.tex <==
\section{Extra-In-Context Learning With Prompts and Bayesian Updating}
Looking at the above exchange, the structure is evident- namely the prompts consist of a sequence of tasks followed by its completion, and the final task is to be completed by the LLM based on the prompts and the original matrix $\tau$ consisting of multinomial probabilities generated by the LLM's training data. Let us denote the sequence of tasks and completions as $(q_k, a_k) \, k=1, \dots, K$ where $a_K$ is to be generated by the LLM. Except for $a_K$, all $(q_k, a_k) \, k=1, \dots, K$, are specified by a sequence of tokens $w_{1,k},w_{2,k},\dots$ that ends with a termination delimiter, typically a new line character.  In this example, $w_{1,k}=\{$, $w_{2,k}='$ for all $k$ while $w_{3,1}=orderby$, $w_{3,4}=groupby$, etc. 

Let the entire sequence of the prompts be denoted by $\mathcal{A}$. 
$a_K$ will be generated using the context window $q_k$ as $w_{1,K}$, $w_{2,K}$ $\dots$ until a termination delimiter is generated. 
Thus, the probability of generating $a_K$ can be written as the product of the corresponding conditional probabilities: 
\begin{equation}
pr_{q_K}\{w_{1,K}|\tau,\mathcal{A}\}pr_{q_K,w_{1,K}}\{w_{2,K}|\tau,\mathcal{A}, w_{1,K}\} pr_{q_K,w_{1,K},w_{2,K}}\{w_{3,K}|\tau,\mathcal{A}, w_{1,K}, w_{2,K}\} \dots
\end{equation}
Each  conditional probability, $pr_c$ is a multinomial probability corresponding to the row $c$ of the matrix. Here $c$ is the context window which goes on changing as new tokens are generated. Now the Bayesian updating can be carried out with the priors specifically defined for each of these conditional probabilities. For example, $a_K$ will give higher posterior probability to $w_{1,K}=\{$, by the Bayesian updating since all $w_{1,k}$ were $\{$. This will be followed by $w_{2,K} = '$, etc. 

Couple of comments are in order
\begin{itemize}
    \item Equation (1), instead of product of multinomial probabilities can be interpreted as multinomial distribution over all possible sequesnce of $w_{i,k}$
\item If the training data corresponding to a particular context window doesn't exist, then, as discussed previously, it can be computed by mapping the context window to the embedding space and then approximated by the multinomial probabilities of the nearby embeddings.
\end{itemize}

To reduce cumbersome notations, we abstract out the above example as a sequence of tasks and their completions $$\, t_1 \rightarrow t_2, t_k \rightarrow t_3, t_k \rightarrow t_3, t_2 \rightarrow t_1, t_k \rightarrow t_1, t_7 \rightarrow t_8, t_{89}\rightarrow t_5,  t_k \rightarrow t_3, \,t_5 \rightarrow t_4 $$
followed by the task $"t_k \rightarrow "$. This entire sequence is $\mathcal{A}$. LLM after learning this sequence, based on In-Context Learning, will  come up with an answer: $' t_{something} '$. Then it will continue to generate the next token, etc. If we examine $\mathcal{A}$, $t_k$ is followed by $t_1$ once and $t_3$ thrice. 

Let $m$ be the total number of possible tokens. For simplicity, let us assume that the row in the matrix corresponding $t_k$'s generative probability has elements $t_i, i=1,...,m$, with the corresponding multinomial probabilities  $P=(p_i, i=1,...,m)$ for some large $m$ based on the LLM training data.  Based on the earlier discussion we will further assume that the prior is Dirichlet distribution ${\mathcal{D}}(p|\alpha_1,\alpha_2,\dots ,\alpha_m)$ with parameters $\alpha_1,\alpha_2,\dots ,\alpha_m$ based on the training data. 

The  posterior distribution of LLM response to $t_k$ for this prompt sequence can be derived as ${\mathcal{D}}(p|\alpha*_1,\alpha*_2,\dots ,\alpha*_m)$, where, $\alpha*_i=\alpha_i$, for $i\neq 1 \, or \,3$. Based on the prompt sequence $\alpha*_1 = \alpha_1 +1$ and $\alpha*_3 = \alpha_3 +3$. Thus, the probability of generating $t_i, i \neq 1 \, or \,3$ is $\alpha_i / (\alpha_+ +4)$, generating $t_1$ is $(\alpha_1+1)/ (\alpha_+ +4) $ and generating $t_3$ is $(\alpha_3+3)/ (\alpha_+ +4) $, where $\alpha_+ = \sum_i \alpha_i$. This process after generation of one of $t_j$'s will continue to generate the next token based on the  conditional  multinomial distribution with the context window $t_j,t_k$, and so on until generation of the termination delimiter. 

We examine the qualitative behavior of the first token generated for this sequence following $t_k$ in the  table below with $\alpha_i =0.3 \,and \, m=10$. As can be observed, with the above prompt sequence, the posterior adjusts to nearly $t_3$ from the pre-trained prior which had all equally likely. 

\begin{table}[h!]
\begin{center}
\begin{tabular}{||c c c ||} 
 \hline
 LLM response to $t_k$ & Pre-Prompt &  Post-Prompt  \\ [0.5ex] 
 \hline\hline
 $t_i, \, i \neq 1 \, or \, 3$ & 0.1 & 0.043  \\ 
 \hline
 $t_1$ & 0.1 & 0.186  \\
 \hline
 $t_3$ & 0.1 & 0.471  \\ 
 \hline
\end{tabular}
\caption{LLM response to $t_k$ with $\alpha_i=0.3$  and $m =10$ }
\label{table:1}
\end{center}
\end{table}

This kind of In-Context learning will continue with the expanded context window and Bayesian updating. One can generalize this development to an arbitrary prior since it can be approximated by a mixture of Dirichlet distributions as described in Section 4. For this case each component of the mixture is Dirichlet and thus it will have similar behavior as described in this section. 


\textbf{New Ideas -ROUGH- But they seem to work}

\textbf{Comment:  The version below uses probabilities for decomposition, but, generation as described is deterministic. However, I think I can change to replace it at token level. Not sure how this will work for general prompts other than our examples} 

\textit{Main Idea}: Decompose $Q$ in mutually exclusive components of the prompts and then use the corresponding subset of their answers to construct our $A$

==> bayesian_LLM_updating_imported.tex <==
\section{Bayesian LLM Updating}
Consider an LLM with a large training data consisting of a variety of clusters or topics including Protein, Love, Poems, Equations, code, etc. Each topic will have different weightings for each token in the vocabulary. As pointed out in Section 2.2, protein cluster\todo[]{We introduce this notion of cluster here. In 2.2 we only talk of a prompt or a prefix} will have higher probability for "shake" and "synthesis" and lower probability for "love". For a given prompt LLM will operate a multinomial probability distribution which would be different for different clusters\todo[]{again, not clear what we mean by clusters - is it prompts/prefixes?}. So in essence, from a Bayesian perspective, there is a prior $u$ which will give different probabilities to different set of clusters and each cluster will have corresponding related terms. As shown in the Dirichlet approximation section any such $u$ can be approximated by a mixture of Dirichlet distributions. The proof was based on a specific construction. So in general we can assume that the LLM represents the prior as
\begin{equation}
u(P)=\sum_{k=1}^{n} a_{k,n}\mathcal{D}((p_1,p_2,\dots,p_m)|((\alpha_{k,1},\alpha_{k,2},\dots,\alpha_{k,m}))
\end{equation}
where, $m$ is the vocabulary size.\todo[]{What is "P"? The prompt?} \\
The above equation makes the relationship between different multinomials and clusters explicit, namely that the LLM is a mixture of $n$ clusters of different Dirichlet priors over the corresponding multinomials with weights $(\alpha_{k,1},\alpha_{k,2},\dots,\alpha_{k,m})$ depending upon the $k^{th}$ cluster and the $k^{th}$ cluster has weight $a_{k,n}$

Let us consider the case of one prompt, say $j*$. It can be shown that the joint probability of $P$ and $j*$, marginal probability of $j*$ and the posterior distribution given $j*$ are given by
\begin{equation}
    u(P, j*)=N, Pr(j*)=D, \,and \, consequently \, u(P|j*)=N/D
\end{equation}
where, 

\begin{align*}
N = \sum_{k=1}^{n}  a_{k,n} (\left \frac{\alpha_{k,j*}}{\sum_{j=1}^m \alpha_{k,j}}\right) \\
&\times \mathcal{D}((p_1,\dots p_{j*-1},p_{j*},p_{j*+1}\dots,p_m)| \\(\alpha_{k,1},\dots \alpha_{k,j*-1}, \\
&  \alpha_{k,j*}+1, \alpha_{k,j*+1}\dots,\alpha_{k,m})
\end{align*}
and, $D$, the marginal probability of $j*$, is obtained by integrating out $P$ from $N$, that is
\begin{align*}
    D= \sum_{k=1}^{n}  a_{k,n} (\left \frac{\alpha_{k,j*}}{\sum_{j=1}^m \alpha_{k,j}}\right)
\end{align*}

For the next prompt, the calculation is obtained iteratively. 

Clearly, 
\begin{enumerate}
    \item The posterior is also a mixture of Dirichlet and it always uses training data for future prompts but it is modified in two ways. 
    \item The corresponding $/alpha_j*$ for each cluster is increased by 1 and all other $/alpha$'s have not changed. That is given the prompt $j*$, the LLM has learnt that term as observed in the discussion on In-Context Learning. 
    \item Most importantly, the mixing coefficients are also changed in such a way that coefficient $a_{k,n}$ is changed by the amount proportional to $\alpha_{k,j*}$. Thus, the posterior gives relatively more weights to the distributions that have higher probability of $j*$
\end{enumerate}

Let us now consider the example of protein, shake and synthesis of Section 2. As soon as the prompt \textit{protein} is received by the LLM, it will  increase the relative weight for selecting those clusters \todo[]{again my confusion of what is a "cluster"?} that have higher probability of having the word \textit{protein}. Since now the \textit{protein} is more prominent,  the token \textit{shake} and \textit{synthesis}, will also be more likely. If the next prompt is \textit{shake}, then by the same reasoning the tokens related to \textit{gym equipment} will be more likely compared to \textit{chemicals}. 

So in effect, the bayes updating here is creating a hierarchical model with soft hierarchy. With the prompt \textit{protein} the probability of cluster corresponding to the token \textit{love} will go down, but it will not be 0, as long as \textit{love} has shown up in the training data. 

For typical LLM, the training data contains many cluster of co-occuring tokens, and thus, the number of terms in the mixture $n$ is likely to be very large. (Vishal- pls check this). GPT-4 has 50,000 tokens in its vocabulary, and suppose $n=100,000$. Then the number of paramters of the Bayesian model will be $99,999 \times 50,000 \approx 5 \, billion$ parameters. \todo[]{why? it is not clear to me why the number of parameters is a product of $n$ (the number of tokens) and the vocabulary}

(Vishal: Do we want to talk about training this model will involve solving a large number of non-linear equations, and that the current state of art models may be doing this by transformer encoder model with attention, but there may other architectures which may be suggested by the Bayesian view. Also need to connect up with The Matrix- it will consist of $50,000^{8,192}$ \todo[]{I am completely confused by what you mean by "cluster". What is it? How are they formed during traiing? What is the relationship of this cluster as the prior and the linear approximation theorem we have earlier?}. Would this be the number of cluster? What $n$ will approximate these many rows of the matrix). 






==> embeddings_algebra.tex <==

\section{Embeddings algebra}\label{sec:embeddings-algebra}
In this section we now return to embeddings and explain the working of LLMs in full generality, not restricted to in-context learning. In Figure~\ref{fig:query_vectors_and_embeddings} we depict in an abstract sense the embeddings that the LLM works with - they consist of both the embeddings of the prompt, as it is introduced token by token, as well as the embeddings of the pre-trained model. In the algorithm for decomposing $Q$, we obtained ${q^*}_1= \argmax_i P(q_i|Q)$. This $\argmax$ operator can be thought of in the embedding space as the embedding closest to $Q$ as a linear combination of pre-trained embeddings as well embeddings of the substrings of the prompt, and utilizing Theorem~\ref{thm:continuity} the next token distribution is obtained from  the linear combination of the distributions. For the pre-trained embeddings, the distribution would be the usual multinomial with probabilities $\{p_1,\dots, p_m\}$, whereas for the substrings of the prompt, the distribution would be $p_i = 1$ at the exact next token of the substring of the prompt, and zero elsewhere.
 

In the case of in-context learning where the prompt is unlikely to be part of the pre-training set, the $\argmax$ operator or the linear combination corresponding to the closest embedding would be dominated by some substring of the prompt which contained the query (as per Assumption 1). For instance, in the example of Table~\ref{tab:queries_outputs}, the whole prompt including the query is the following: 
{\textit{Tournament0 team with best win loss record after losing the toss
\{'orderby': ['win\_loss\_\{ratio'], 'toss': ['lost'], 'tournament': ['Tournament0'], 'type': ['team']\}
lowest team total
\{'groupby': ['innings'], 'orderby': ['runs'], 'sortorder': ['reverse'], 'type': ['team']\}
biggest Tournament0 total in defeat
\{'groupby': ['innings'], 'orderby': ['runs'], 'result': ['loss'], 'tournament': ['Tournament0'], 'type': ['team']\}
highest scores by Team0
\{'groupby': ['innings'], 'orderby': ['runs'], 'team': ['Team0'], 'type': ['team']\}
highest losing team total in Tournament0}}

The new query $Q$ is the last part \textit{highest losing team total in Tournament0}, and the closest embedding vector to that would be the substring which ends in \textit{biggest Tournament0 total in defeat} and whatever came before it (prefix) (so $q_3$+prefix in this case). The LLM would then construct a distribution by a combination of the embedding of ($q_3$+prefix) and whatever is residual between the prompt and ($q_3$+prefix) and this distribution would be dominated by the empirical next token distribution of ($q_3$+prefix) which is $a_3$. This process continues token by token and the completion generated.


In case of a generic completion, the linear combination would likely be dominated by the pre-trained set (as our New York Times example demonstrated) unless we introduce the deliberate ``Fed Chairman Ramesh K Sitaraman'' which affects the distribution the next time anything related to the Fed chairman needs to be generated and Ramesh K Sitaraman is repeated. This ability to learn from the prompt on the fly, even outside of in-context learning, contributes significantly to the success and human like quality of modern LLM based chatbots.



\begin{figure}[htbp]
\centering
\begin{tikzpicture}[scale=1.2]
% Define the text strings
\def\textAFull{Tournament0 team with best win loss record after losing the toss}
\def\textAShort{Tournament0 team ... toss}
\def\textB{{'orderby': ... ['team']}}
\def\textC{lowest ... total}
\def\textD{{'groupby': ... ['team']}}
\def\textE{biggest ... defeat}
\def\textF{{'groupby': ... ['team']}}
\def\textG{highest ... Team0}
\def\textH{{'groupby': ... ['team']}}

% Draw query vectors with labels
\foreach \offset/\angle/\label [count=\i] in {
    0/0/\textAFull,
    0.3/-2/\textAShort\textB,
    0.6/-4/\textAShort\textB\textC,
    0.9/-6/\textAShort\textB\textC\textD,
    1.2/-8/\textAShort\textB\textC\textD\textE,
    1.5/-10/\textAShort\textB\textC\textD\textE\textF,
    1.8/-12/\textAShort\textB\textC\textD\textE\textF\textG,
    2.1/-14/\textAShort\textB\textC\textD\textE\textF\textG\textH
} {
    \draw[->, thick, blue] (\offset, {-0.7*\i}) -- ++(\angle:5);
    \path[postaction={decorate,decoration={text along path,text align=center,text={|\tiny|\label}, raise=3pt}}]
        ({\offset+0.2*cos(\angle)}, {-0.7*\i+0.2*sin(\angle)}) -- ++({\angle}:4.6);
    \node[circle, fill=black, inner sep=1pt] at ({\offset + 5*cos(\angle)}, {-0.7*\i + 5*sin(\angle)}) {};
    \node[font=\scriptsize] at ({\offset + 5.2*cos(\angle)}, {-0.7*\i + 5.2*sin(\angle)}) {\i};
}

% Draw pre-trained embedding vectors
\foreach \x/\y/\angle [count=\i] in {
    -1.5/-2/30, -1/-2.5/45, -0.5/-3/60, 0/-3.5/40, 0.5/-4/50, 1/-4.5/35,
    1.5/-5/55, -1.2/-5.5/25, -0.8/-6/65, 0.2/-6.5/70, 0.8/-7/20, 1.2/-7.5/75,
    2.5/-2/150, 3/-2.5/135, 3.5/-3/120, 4/-3.5/140, 3.5/-4/130, 3/-4.5/145,
    2.5/-5/125, 3.2/-5.5/155, 3.8/-6/115, 2.8/-6.5/110, 3.2/-7/160, 3.8/-7.5/105
} {
    \draw[->, thick, red!30, opacity=0.3] (\x,\y) -- ++(\angle:3);
    \path[red!30, opacity=0.3, postaction={decorate,decoration={text along path,text align=center,text={|\tiny|pre-trained \i}, raise=2pt}}]
        ({\x+0.2*cos(\angle)}, {\y+0.2*sin(\angle)}) -- ++(\angle:2.6);
}
\end{tikzpicture}
\caption{Vector representation of progressive query substrings and pre-trained embeddings}
\label{fig:query_vectors_and_embeddings}
\end{figure}
